Can LLMs plan paths with extra hints from solvers?

Large Language Models (LLMs) have shown remarkable capabilities in natural language processing, mathematical problem solving, and tasks related to program synthesis. However, their effectiveness in long-term planning and higher-order reasoning has been noted to be limited and fragile. This paper explores an approach for enhancing LLM performance in solving a classical robotic planning task by integrating solver-generated feedback. We explore four different strategies for providing feedback, including visual feedback, we utilize fine-tuning, and we evaluate the performance of three different LLMs across a 10 standard and 100 more randomly generated planning problems. Our results suggest that the solver-generated feedback improves the LLM's ability to solve the moderately difficult problems, but the harder problems still remain out of reach. The study provides detailed analysis of the effects of the different hinting strategies and the different planning tendencies of the evaluated LLMs.

==> appendices.tex <==
\section{Appendix}
\subsection{Prompting details}
\label{sec:prompt_details}

The initial prompt for explaining the path planning problem is as follows:

\begin{verbatim}
    We are going to solve ... 
\end{verbatim}

\subsection{Other tables}
\subsubsection{}
\begin{table*}[h!]
\centering
\begin{tabular}{ccc}
\toprule
\textbf{Environment} & \textbf{Result} & \textbf{Success Rate}  \\ \midrule
\multicolumn{3}{c}{\textbf{Solvable Versions}} \\ \midrule
\textbf{Box}          & 10 Correct & 100\% \\
\textbf{Box Boundary} & 10 Correct & 100\% \\
\textbf{Canyon}       & 9 Correct &  90\% \\
\textbf{Curve}        & 8 Correct &  80\% \\
\textbf{Diagonal Wall}& 10 Correct & 100\% \\
\textbf{Easy}         & 10 Correct & 100\% \\
\textbf{Maze 2D}      & 8 Correct &  80\% \\
\textbf{Scots HSCC16} & 8 Correct &  80\% \\
\textbf{Spiral}       & 9 Correct &  90\% \\
\textbf{Wall}         & 10 Correct & 100\% \\ \midrule
\multicolumn{3}{c}{\textbf{Unsolvable Versions}} \\ \midrule
\textbf{Box}          & 10 Incorrect & 0\% \\
\textbf{Box II}       & 10 Incorrect & 0\% \\
\textbf{Canyon}       & 10 Incorrect & 0\% \\
\textbf{Curve}        & 1 Correct, 9 Incorrect & 10\% \\
\textbf{Diagonal Wall}& 10 Incorrect & 0\% \\
\textbf{Easy}         & 10 Incorrect & 0\% \\
\textbf{Maze 2D}      & 10 Incorrect & 0\% \\
\textbf{Scots HSCC16} & 1 Correct, 9 Incorrect & 10\% \\
\textbf{Spiral}       & 1 Correct, 9 Incorrect & 10\% \\
\textbf{Wall}         & 10 Incorrect & 0\% \\ \midrule
\textbf{Average}      & \multicolumn{2}{c}{Solvable: 92.00\% Correct} \\
\textbf{Average}      & \multicolumn{2}{c}{Unsolvable: 3.00\% Correct} \\
\bottomrule
\end{tabular}
\caption{Experiment: Identify solvable or not. Model: llama-3.1-70b-versatile. Prompting strategy: solvable\_prompt.}
\label{table:results2}
\end{table*}


\begin{figure*}
    \centering


\begin{table}[H]
\centering
\begin{tabular}{lccccccccc}
\toprule
\textbf{Problem} & \multicolumn{3}{c}{\textbf{Gemini Pro 1.5}} & \multicolumn{3}{c}{\textbf{GPT-4o}} & \multicolumn{3}{c}{\textbf{Claude Sonnet 3.5}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}              
                    & \textbf{S\%} & \textbf{N} & \textbf{PL} 
                    & \textbf{S\%} & \textbf{N} & \textbf{PL Succ.} 
                    & \textbf{S\%} & \textbf{N} & \textbf{PL} \\ 
\midrule
\textbf{Box}             & 90  & 8.80  & 6.33  & 50\%  & 17.30 & 8.00  & 30  & 17.33 & 5.00  \\ 
\textbf{Box B.}    & 100 & 1.30  & 3.70  & 100\% & 1.00  & 3.90  & 100 & 1.20  & 4.10  \\ 
\textbf{Canyon}          & 30  & 15.90 & 5.33  & 100\% & 2.60  & 4.60  & 80  & 5.62  & 5.88  \\ 
\textbf{Curve}           & 30  & 17.90 & 11.00 & 100\% & 4.30  & 5.80  & 20  & 16.50 & 8.50  \\ 
\textbf{D. Wall}   & 90  & 8.90  & 7.78  & 0\%   & 20.00 & -     & 0   & -     & -     \\ 
\textbf{Easy}            & 100 & 3.90  & 6.60  & 100\% & 6.40  & 5.60  & 20  & 12.50 & 6.00  \\ 
\textbf{Maze}            & 10  & 20.10 & 13.00 & 0\%   & 20.00 & -     & 0   & -     & -     \\ 
\textbf{Scots}           & 0   & -     & -     & 10\%  & 18.70 & 10.00 & 0   & -     & -     \\ 
\textbf{Spiral}          & 30  & 17.10 & 9.00  & 0\%   & 20.00 & -     & 0   & -     & -     \\ 
\textbf{Wall}            & 100 & 8.00  & 6.50  & 100\% & 5.40  & 6.90  & 10  & 20.00 & 7.00  \\ 
\midrule
\textbf{1 Obs}      & 100 & 1.90  & 4.80  & 70\%  & 1.86  & 5.14  & 55  & 2.18  & 4.45  \\ 
\textbf{2 Obs}     & 60  & 2.83  & 6.33  & 50\%  & 2.60  & 5.50  & 35  & 1.43  & 4.14  \\ 
\textbf{3 Obs}     & 65  & 4.15  & 6.77  & 20\%  & 2.25  & 6.25  & 20  & 3.25  & 5.75  \\ 
\textbf{4 Obs}     & 20  & 5.00  & 7.50  & 10\%  & 5.50  & 9.00  & 10  & 2.00  & 4.00  \\ 
\textbf{5 Obs}     & 35  & 3.86  & 6.86  & 15\%  & 3.00  & 7.00  & 15  & 5.33  & 6.00  \\ 
\bottomrule
\end{tabular}
\caption{Comparison of performance metrics across different environments for Gemini Pro 1.5, GPT-4o, and Claude Sonnet 3.5.}
\label{table:merged_results}
\end{table}




\begin{table}[H]
\centering
\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{\textbf{Gemini Pro 1.5}} & \multicolumn{3}{c}{\textbf{GPT-4o}} & \multicolumn{3}{c}{\textbf{Claude Sonnet 3.5}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}              
                    \textbf{Problem} & \textbf{Success R.} & \textbf{Iter. Succ.} & \textbf{PL Succ.} 
                    & \textbf{Success R.} & \textbf{Iter. Succ.} & \textbf{PL Succ.} 
                    & \textbf{Success R.} & \textbf{Iter. Succ.} & \textbf{PL Succ.} \\ 
\midrule
\textbf{Easy}            & 100\% & 3.90  & 6.60  & 100\% & 6.40  & 5.60  & 20\%  & 12.50 & 6.00  \\ 
\textbf{Box B.}    & 100\% & 1.30  & 3.70  & 100\% & 1.00  & 3.90  & 100\% & 1.20  & 4.10  \\ 
\textbf{Wall}            & 100\% & 8.00  & 6.50  & 100\% & 5.40  & 6.90  & 10\%  & 20.00 & 7.00  \\ 
\textbf{Box}             & 90\%  & 8.80  & 6.33  & 50\%  & 17.30 & 8.00  & 30\%  & 17.33 & 5.00  \\ 
\textbf{Canyon}          & 30\%  & 15.90 & 5.33  & 100\% & 2.60  & 4.60  & 80\%  & 5.62  & 5.88  \\ 
\textbf{D. Wall}   & 90\%  & 8.90  & 7.78  & 0\%   & 20.00 & -     & 0\%   & -     & -     \\ 
\textbf{Curve}           & 30\%  & 17.90 & 11.00 & 100\% & 4.30  & 5.80  & 20\%  & 16.50 & 8.50  \\ 
\textbf{Spiral}          & 30\%  & 17.10 & 9.00  & 0\%   & 20.00 & -     & 0\%   & -     & -     \\ 
\textbf{Maze}            & 10\%  & 20.10 & 13.00 & 0\%   & 20.00 & -     & 0\%   & -     & -     \\ 
\textbf{Scots}           & 0\%   & -     & -     & 10\%  & 18.70 & 10.00 & 0\%   & -     & -     \\ 
\midrule
\textbf{1 Obs}      & 100\% & 1.90  & 4.80  & 70\%  & 1.86  & 5.14  & 55\%  & 2.18  & 4.45  \\ 
\textbf{2 Obs}     & 60\%  & 2.83  & 6.33  & 50\%  & 2.60  & 5.50  & 35\%  & 1.43  & 4.14  \\ 
\textbf{3 Obs}     & 65\%  & 4.15  & 6.77  & 20\%  & 2.25  & 6.25  & 20\%  & 3.25  & 5.75  \\ 
\textbf{4 Obs}     & 20\%  & 5.00  & 7.50  & 10\%  & 5.50  & 9.00  & 10\%  & 2.00  & 4.00  \\ 
\textbf{5 Obs}     & 35\%  & 3.86  & 6.86  & 15\%  & 3.00  & 7.00  & 15\%  & 5.33  & 6.00  \\ 
\bottomrule
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\begin{tabular}{lccccccccc}
\toprule
& \multicolumn{3}{c}{\textbf{Gemini}} & \multicolumn{3}{c}{\textbf{GPT-4o}} & \multicolumn{3}{c}{\textbf{Claude}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}              
\textbf{Problem} & \textbf{SR\%} & \textbf{IS} & \textbf{PL} 
                    & \textbf{SR\%} & \textbf{IS} & \textbf{PL} 
                    & \textbf{SR\%} & \textbf{IS} & \textbf{PL} \\ 
\midrule
\textbf{Easy}            & 100 & 3.9  & 6.6  & 100 & 6.4  & 5.6  & 20 & 12.5 & 6.0  \\ 
\textbf{Box B.}    & 100 & 1.3  & 3.7  & 100 & 1.0  & 3.9  & 100 & 1.2  & 4.1  \\ 
\textbf{Wall}            & 100 & 8.0  & 6.5  & 100 & 5.4  & 6.9  & 10 & 20.0 & 7.0  \\ 
\textbf{Box}             & 90 & 8.8  & 6.3  & 50  & 17.3 & 8.0  & 30 & 17.3 & 5.0  \\ 
\textbf{Canyon}          & 30  & 15.9 & 5.3  & 100 & 2.6  & 4.6  & 80 & 5.6  & 5.9  \\ 
\textbf{D. Wall}   & 90  & 8.9  & 7.8  & 0   & 20.0 & -     & 0  & -     & -     \\ 
\textbf{Curve}           & 30  & 17.9 & 11.0 & 100 & 4.3  & 5.8  & 20 & 16.5 & 8.5  \\ 
\textbf{Spiral}          & 30  & 17.1 & 9.0  & 0   & 20.0 & -     & 0  & -     & -     \\ 
\textbf{Maze}            & 10  & 20.1 & 13.0 & 0   & 20.0 & -     & 0  & -     & -     \\ 
\textbf{Scots}           & 0   & -     & -     & 10  & 18.7 & 10.0 & 0  & -     & -     \\ 
\midrule
\textbf{1 Obs}      & 100 & 1.9  & 4.8  & 70  & 1.9  & 5.1  & 55 & 2.2  & 4.5  \\ 
\textbf{2 Obs}     & 60  & 2.8  & 6.3  & 50  & 2.6  & 5.5  & 35 & 1.4  & 4.1  \\ 
\textbf{3 Obs}     & 65  & 4.2  & 6.8  & 20  & 2.3  & 6.3  & 20 & 3.3  & 5.8  \\ 
\textbf{4 Obs}     & 20  & 5.0  & 7.5  & 10  & 5.5  & 9.0  & 10 & 2.0  & 4.0  \\ 
\textbf{5 Obs}     & 35  & 3.9  & 6.9  & 15  & 3.0  & 7.0  & 15 & 5.3  & 6.0  \\ 
\bottomrule
\end{tabular}
\end{table}



\end{figure*}


\begin{itemize}

    \item \textcolor{red}{Gemini 1.5 pro}
    \begin{table}[H]
    \centering
    \begin{tabular}{lcccccc}
    \toprule
    \textbf{Environment}     & \textbf{Success R.} & \textbf{Iter. Succ.} & \textbf{Path Len.} & \textbf{PL Succ.} \\ 
    \midrule
    \textbf{Box}             & 90\%             & 10.89               & 4.50               & 4.44              \\ 
    \textbf{Box Boundary}    & 100\%            & 1.30                & 3.70               & 3.70              \\ 
    \textbf{Canyon}          & 0\%              & -                   & 4.90               & -                 \\ 
    \textbf{Curve}           & 40\%             & 8.00                & 5.50               & 6.50              \\ 
    \textbf{Diagonal Wall}   & 70\%             & 8.86                & 4.90               & 5.00              \\ 
    \textbf{Easy}            & 100\%            & 3.30                & 4.50               & 4.50              \\ 
    \textbf{Maze 2D}         & 0\%              & -                   & 6.80               & -                 \\ 
    \textbf{Scots HSCC16}    & 20\%             & 13.50               & 14.40              & 12.50             \\ 
    \textbf{Spiral}          & 60\%             & 14.17               & 6.10               & 6.17              \\ 
    \textbf{Wall}            & 100\%            & 1.60                & 4.20               & 4.20              \\ 
    \midrule
    \textbf{1 Obstacle} & 95\% & 1.74 & 4.25 & 4.11 \\
    \textbf{2 Obstacles} & 95\% & 2.53 & 4.90 & 4.89 \\
    \textbf{3 Obstacles} & 75\% & 2.87 & 5.30 & 4.87 \\
    \textbf{4 Obstacles} & 45\% & 3.67 & 5.45 & 4.89 \\
    \textbf{5 Obstacles} & 30\% & 3.67 & 5.70 & 4.83 \\
        
    \bottomrule
    \end{tabular}
    \caption{Man runtime: 03h:33m:23s, Random runtime:  01h:01m:23s}
    \label{table:results_summary1}
    \end{table}




    \item GPT-4o (add random table (gpt\_full\_path)
    \begin{table}[H]
    \centering
    \begin{tabular}{lcccccc}
    \toprule
    \textbf{Environment} & \textbf{Success R.} & \textbf{Iter. Succ.} & \textbf{Path Len.} & \textbf{PL Succ.} \\ 
    \midrule
    \textbf{Box}             & 50\%             & 8.60               & 4.90               & 5.20              \\ 
    \textbf{Box Boundary}    & 100\%            & 1.00               & 3.00               & 3.00              \\ 
    \textbf{Canyon}          & 100\%            & 2.20               & 4.70               & 4.70              \\ 
    \textbf{Curve}           & 70\%             & 9.14               & 5.60               & 5.43              \\ 
    \textbf{Diagonal Wall}   & 0\%              & -              & 4.60               & -1.00             \\ 
    \textbf{Easy}            & 100\%            & 2.60               & 5.20               & 5.20              \\ 
    \textbf{Maze 2D}         & 0\%              & -              & 6.60               & -1.00             \\ 
    \textbf{Scots HSCC16}    & 0\%              & -              & 9.10               & -1.00             \\ 
    \textbf{Spiral}          & 0\%              & -              & 5.30               & -1.00             \\ 
    \textbf{Wall}            & 100\%            & 1.60               & 4.50               & 4.50              \\ 
    \midrule
    \textbf{1 Obstacle} & 90.00\% & 1.67 & 5.15 & 4.94 \\
    \textbf{2 Obstacles} & 50.00\% & 2.30 & 6.95 & 5.70 \\
    \textbf{3 Obstacles} & 15.00\% & 4.00 & 7.10 & 6.33 \\
    \textbf{4 Obstacles} & 5.00\%  & 1.00 & 8.00 & 5.00 \\
    \textbf{5 Obstacles} & 10.00\% & 3.00 & 7.80 & 7.00 \\
    \bottomrule
    \end{tabular}
    \caption{Max iterations: 20, Runtime: 02h:50m:27s; Number of iterations: 5, Evaluations per Env: 20, Runtime: 01h:13m:09s}
    \label{table:results_summary2}
    \end{table}






\item{Claude 3.5}
\begin{table}[H]
\centering
\begin{tabular}{lcccccc}
\toprule
\textbf{Environment} & \textbf{Success R.} & \textbf{Iter. Succ.} & \textbf{Path Len.} & \textbf{PL Succ.} \\ 
\midrule
\textbf{Box}             & 0\%              & -              & 4.60               & -1.00             \\ 
\textbf{Box Boundary}    & 100\%            & 1.00               & 3.60               & 3.60              \\ 
\textbf{Canyon}          & 70\%             & 7.14               & 5.90               & 5.71              \\ 
\textbf{Curve}           & 10\%             & 3.00               & 12.60              & 9.00              \\ 
\textbf{Diagonal Wall}   & 0\%              & -              & 4.60               & -1.00             \\ 
\textbf{Easy}            & 0\%              & -              & 4.40               & -1.00             \\ 
\textbf{Maze 2D}         & 0\%              & -              & 16.40              & -1.00             \\ 
\textbf{Scots HSCC16}    & 0\%              & -              & 11.60              & -1.00             \\ 
\textbf{Spiral}          & 0\%              & -              & 4.50               & -1.00             \\ 
\textbf{Wall}            & 10\%             & 11.00              & 5.10               & 5.00              \\ 
\midrule
\textbf{1 Obstacle} & 85.00\% & 1.94 & 4.65 & 4.53 \\
\textbf{2 Obstacles} & 60.00\% & 1.75 & 5.05 & 4.33 \\
\textbf{3 Obstacles} & 25.00\% & 3.40 & 5.50 & 4.60 \\
\textbf{4 Obstacles} & 0.00\%  & -1.00 & 6.15 & -1.00 \\
\textbf{5 Obstacles} & 15.00\% & 3.00 & 6.45 & 5.00 \\
\bottomrule
\end{tabular}
\caption{Max iterations: 20, Runtime comparison of random environments and manual settings.}
\end{table}



\end{itemize}


% \paragraph{Free form Quadrilaterals *}
% \textcolor{red}{Gemini Pro 1.5}:

% \begin{table}[H]
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Environment} & \textbf{Success R.} & \textbf{Iter. Succ.} & \textbf{Path Len.} & \textbf{PL Succ.} \\ 
% \midrule
% \textbf{Box}                 & 90\% & 8.80  & 6.10  & 6.33  \\ 
% \textbf{Box Boundary}        & 100\% & 1.30  & 3.70  & 3.70  \\ 
% \textbf{Canyon}              & 30\% & 15.90 & 5.50  & 5.33  \\ 
% \textbf{Curve}               & 30\% & 17.90 & 9.00  & 11.00 \\ 
% \textbf{Diagonal Wall}       & 90\% & 8.90  & 7.40  & 7.78  \\ 
% \textbf{Easy}                & 100\% & 3.90  & 6.60  & 6.60  \\ 
% \textbf{Maze}                & 10\% & 20.10 & 8.70  & 13.00 \\ 
% \textbf{Scots}               & 0\%  & - & 8.70  & -     \\ 
% \textbf{Spiral}              & 30\% & 17.10 & 7.50  & 9.00  \\ 
% \textbf{Wall}                & 100\% & 8.00  & 6.50  & 6.50  \\ 
% \midrule
% \textbf{1 Obstacle}   & 100\% & 1.90  & 4.80  & 4.80  \\ 
% \textbf{2 Obstacles}  & 60\%  & 2.83  & 6.25  & 6.33  \\ 
% \textbf{3 Obstacles}  & 65\%  & 4.15  & 7.05  & 6.77  \\ 
% \textbf{4 Obstacles}  & 20\%  & 5.00  & 6.60  & 7.50  \\ 
% \textbf{5 Obstacles}  & 35\%  & 3.86  & 7.05  & 6.86  \\ 
% \bottomrule
% \end{tabular}
% \caption{Total runtime: 04h:36m:18s, TOTAL
% RUNTIME Random: 01H:09M:23S}
% \label{table:Gemini_all_Envs}
% \end{table}

% GPT 4o:
% \begin{table}[H]
%     \centering
%     \begin{tabular}{lcccccc}
%     \toprule
%     \textbf{Environment}     & \textbf{Success R.} & \textbf{Iter. Succ.} & \textbf{Path Len.} & \textbf{PL Succ.} \\ 
%     \midrule
%     \textbf{Box}             & 50\%             & 17.30               & 8.00               & 8              \\ 
%     \textbf{Box Boundary}    & 100\%            & 1.00                & 3.90               & 3.90              \\ 
%     \textbf{Canyon}          & 100\%            & 2.60                & 4.60               & 4.60              \\ 
%     \textbf{Curve}           & 100\%            & 4.30                & 5.80               & 5.80              \\ 
%     \textbf{Diagonal Wall}   & 0\%              & 20.00               & 6.60               & -                 \\ 
%     \textbf{Easy}            & 100\%            & 6.40                & 5.60               & 5.60              \\ 
%     \textbf{Maze}            & 0\%              & 20.00               & 10.10              & -                 \\ 
%     \textbf{Scots}           & 10\%             & 18.70               & 8.30               & 10.00             \\ 
%     \textbf{Spiral}          & 0\%              & 20.00               & 7.30               & -                 \\ 
%     \textbf{Wall}            & 100\%            & 5.40                & 6.90               & 6.90              \\ 
%     \midrule
%     \textbf{1 Obstacle}   & 70\%  & 1.86  & 6.05  & 5.14  \\ 
%     \textbf{2 Obstacles}  & 50\%  & 2.60  & 6.40  & 5.50  \\ 
%     \textbf{3 Obstacles}  & 20\%  & 2.25  & 8.25  & 6.25  \\ 
%     \textbf{4 Obstacles}  & 10\%  & 5.50  & 8.30  & 9.00  \\ 
%     \textbf{5 Obstacles}  & 15\%  & 3.00  & 8.10  & 7.00  \\ 
%     \bottomrule
%     \end{tabular}
%     \caption{ Total runtime: 03h:35m:08s, Total runtime:  01H:17M:26S}
%     \label{table:results_gpt_all_envs}
% \end{table}


% Claude Sonnet 3.5:

% \begin{table}[H]
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Environment} & \textbf{Success R.} & \textbf{Iter. Succ.} & \textbf{Path Len.} & \textbf{PL Succ.} \\ 
% \midrule
% \textbf{Box}            & 30\%  & 17.33  & 5.30  & 5.00  \\ 
% \textbf{Box Boundary}   & 100\% & 1.20   & 4.10  & 4.10  \\ 
% \textbf{Canyon (regular)}         & 80\%  & 5.62   & 6.10  & 5.88  \\ 
% \textbf{Curve (regular)}          & 20\%  & 16.50  & 9.50  & 8.50  \\ 
% \textbf{Diagonal Wall}  & 0\%   & -      & 5.50  & -     \\ 
% \textbf{Easy (regular)}           & 20\%  & 12.50  & 6.40  & 6.00  \\ 
% \textbf{Maze 2D}        & 0\%   & -      & 9.30  & -     \\ 
% \textbf{Scots HSCC16}   & 0\%   & -      & 6.00  & -     \\ 
% \textbf{Spiral}         & 0\%   & -      & 5.80  & -     \\ 
% \textbf{Wall}           & 10.00\%  & 20.00  & 6.50  & 7.00  \\ 
% \midrule
% \textbf{1 Obstacle}   & 55\%  & 2.18  & 5.05  & 4.45  \\ 
% \textbf{2 Obstacles}  & 35\%  & 1.43  & 5.10  & 4.14  \\ 
% \textbf{3 Obstacles}  & 20\%  & 3.25  & 6.00  & 5.75  \\ 
% \textbf{4 Obstacles}  & 10\%  & 2.00  & 6.25  & 4.00  \\ 
% \textbf{5 Obstacles}  & 15\%  & 5.33  & 5.90  & 6.00  \\ 
% \bottomrule
% \end{tabular}
% \caption{ Total time: 02h:28m:58s., 00H:33M:35S}
% \label{table:results_summary}
% \end{table}

==> dm.tex <==
Input: $\tau = \{\langle p_i, t_i \rangle\}, r_s, \{\ell_i\}$
        $p_c = \mathit{intersect}(\tau,\{\ell_i\})$
        if $p_c = \bot$ then output $\mathit{go}$
        else
                $t_c$ time corresp. to $p_c$ in $\tau$
                $B = B(p_c,r_s)$
                $\tau_v = \mathit{simulate}(x,v,t_0,\{\ell_i\})$
                $[t_1,t_2] = \mathit{interTime}(\tau_v,B)$
                if $t_c \in [t_1, t_2]$ 
                        then output $\mathit{brake}$
                else if $t_c \in [t_1-t_s, t_2+t_s]$
                        then output $\mathit{slow}$
                else output $\mathit{go}$
